WhisperFlow: speech foundation models in real time

Speech foundation models, such as OpenAI's Whisper, become the state of the art in speech understanding due to their strong accuracy and generalizability. Yet, their applications are mostly limited to processing pre-recorded speech, whereas processing of streaming speech, in particular doing it efficiently, remains rudimentary. Behind this inefficiency are multiple fundamental reasons: (1) speech foundation models are trained to process long, fixed-length voice inputs (often 30 seconds); (2) encoding each voice input requires encoding as many as 1,500 tokens with tens of transformer layers; (3) decoding each output entails an irregular, complex beam search. As such, streaming speech processing on resource-constrained client devices is more expensive than other AI tasks, e.g., text generation. To this end, we present a novel framework, WhisperFlow, which embodies both model and system optimizations. (1) Hush word as a short, learnable audio segment; appended to a voice input, a hush word gracefully stops the speech model from processing more input without hallucination; (2) Beam pruning, which aligns streaming audio buffers over time and reuses results from earlier decoding rounds, therefore significantly accelerating decoding; and (3) CPU/GPU pipelining, which not only maps to the encoding/decoding stages dynamically, but also tunes to an optimal resource ratio, respecting the encoding/decoding speed that varies across voice inputs, models, and hardware. We test WhisperFlow on commodity ARM platforms with 4-12 CPU cores and 10-30 GPU cores. It reduces per-word latency by 1.6x-4.7x to as low as 0.5 second, while seeing negligible accuracy degradation. On an entry-level MacBook Air, WhisperFlow can keep the per-word latency around 1 second, with the whole device drawing only 7 Watts in total.

==> conclusion.tex <==
\section{Conclusion}


==> design2.tex <==
% !TeX root = main.tex

% \subsection{Hybrid execution speedup and selective offloading }
\section{The offloading path}
\label{sec:design2}

placeholder for design 2 if necessary

==> fig-models.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.48\textwidth]{./figs/models}
	%	\vspace{-2em}
	\caption{Compared to popular encoder-decoder SU models (left), our model (right) shifts much of the encoding computation to bottom layers, allowing them to be executed in a streaming fashion during ingestion.
 XXX show segment by segment input... XXX 
	}
	\label{fig:mo}
	%	\vspace{-5mm}
\end{figure}

==> fig-motivpl.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.45\textwidth]{./figs/motivpl}
	%	\vspace{-2em}
	% \caption{The offloading break down of selective offloading and sampling offloading. Selective offloading can help largely reduce the offloading data count by preventing offload non-target data}
	\caption{The deep SU pipeline~\cite{conformer-2020,peng2022branchformer,baevski2020wav2vec}.
	The input of SU tasks, an 1D raw wavform of the audio, will first go through STFT+Mel filter bank to get spectrum, then processed by encoder to get intermediate encode representation, and finally decoded in an autoregressive fashion by hybrid transformer/CTC decoder coupled with beam search method
	}
	\label{fig:motivpl}
	
	%	\vspace{-5mm}
\end{figure}

==> figs/tmp-pdfcrop-14104.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{64657369676E6265616D7072756E696E672E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}
\page 1 [39 11 728 445]
\csname @@end\endcsname
\end


==> figs/tmp-pdfcrop-14788.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{6532652E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-15844.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{696E74726F2E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-16136.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{696E74726F2E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-17584.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{706970656C696E652E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-1880.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{696E74726F2E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-18812.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{696E74726F2E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-19672.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{653265302E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-20996.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{6D6F746976656E636465632D2D2E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}
\page 1 [89 529 433 720]
\csname @@end\endcsname
\end


==> figs/tmp-pdfcrop-21368.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{6532652E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-21740.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{706970656C696E652E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-26520.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{706970656C696E652E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-26968.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{706970656C696E652E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}
\page 1 [446 1407 2186 2546]
\csname @@end\endcsname
\end


==> figs/tmp-pdfcrop-28152.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{696E74726F2E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-2940.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{696E74726F2E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-31388.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{676C6F73736172792E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}
\page 1 [35 667 514 756]
\csname @@end\endcsname
\end


==> figs/tmp-pdfcrop-32000.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{64657369676E617564696F687573687461672E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}
\page 1 [67 242 778 343]
\csname @@end\endcsname
\end


==> figs/tmp-pdfcrop-34080.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{696E74726F2E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-35460.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{706F7765722E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-36676.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{6532652E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-40812.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{706970656C696E652E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}
\page 1 [446 1450 2186 2603]
\csname @@end\endcsname
\end


==> figs/tmp-pdfcrop-40820.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{696E74726F2E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-40920.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{696E74726F2E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-44368.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{70696C6F74737065656475702E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}
\page 1 [90 633 437 721]
\csname @@end\endcsname
\end


==> figs/tmp-pdfcrop-7728.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{696E74726F2E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> figs/tmp-pdfcrop-9408.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{706970656C696E652E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> motiv__Felix_s_conflicted_copy_2024-11-25_.tex <==
\section{Motivations}
\label{sec:motiv}

\subsection{Speech foundation models}


For the past several decades, ASR has been a key AI task, with rsarch methodologies evolving from traditional signal processing~\cite{davis1952automatic} to Hidden Markov models (HMM) ~\cite{Baker1975HMM} to modern deep learning approaches ~\cite{hori2017advances, peng2022branchformer, kim2024convolution}. 

\textit{Foundation speech models}, as exmeplfied by OpenAI’s Whisper~\cite{radford2023robust}, are encoder-decode rtransofmers. 
They are trained on massive datasets (e.g. 960K hours),
are XXX larger than the models before them (often XXX hours) and
The most notable benefit of the foundation models is their generalizability capabijliity: 
they deliver storng accuracy on unseen datasets(e.g. new languages, accents, and challenging real-world conditions) -- without finetuning on these datasets. 
This constarsts to classic models; and also makes them the top cjioce for today's speech unerastnding systms. 


\subsection{SSP with speech foundation models}

\xzlNote{two paragraphs below should be ocmpressed}
\xzlNote{should integrate with a figure. maybe figure 1}

SSP is traditionally done with RNN models: as RNN models, by construciotn, can operate on partial audio input and generate partial transcript output. 
However, lacking complete audio contexts, such RNN models often reulst in signicant word errors. As a remedy ... \xzlNote{RW complete}. 



For instance, the Whisper-streaming system \cite{machavcek2023turning} manages streaming audio by periodically updating an audio and transcript buffer, shown in ~\autoref{fig:intro} (b). With techniques like LocalAgreement-2 \cite{Liu2020LowLatencySS}, transcripts are confirmed after repetition, and the audio buffer and prompt are dynamically adjusted to maintain alignment and buffer length for accurate, low-latency processing.

\xzlNote{mege here?}
attempting to feed the model with shorter inputs (i.e., with less padding) will cause it to hallucinate and produce gibberish, shown in prior discussion~\cite{ggerganov2022streamdiscussion} and by us (Section~\ref{sec:motiv}). 


%Applying speech foundation models into SSP task is quite natural idea, as the system can benefit from the foundation models' generalizability. However, the existing foundation models are not designed for such tasks. specific model serving system with dedicated design is required. To this end, state-of-the-art system has been proposed to serve the speech foundation models for SSP tasks . Take the whisper-streaming system ~\cite{machavcek2023turning} as an example. it takes the streaming audio input periodically, holds an audio buffer and a transcript buffer. With LocalAgreement-2~\cite{Liu2020LowLatencySS}, the transcript will be confirmed after occurred 2 times. Based on the progress, the audio buffer and the prompt will be updated, to keep the audio buffer around a certain length, and the prompt align with the audio buffer. 

The aforementioned system is designed for operating on devices with good GPU, and purely operate on GPU to deliver low latency and high accuracy. It treat the Whisper model as a simple API that transcribe the audio to text. However, we notice that there are significant inefficiency in the current system. We will elaborate this in the following sections.


\subsection{The computation redundancy}
One major perspective of inefficiencies in the current system is the redundancy in the computation among the whole process. 

\xzlNote{should integrate with figure. maybe figure 1.}
the analysis can also be better, e.g. using GFLOPS, under typical input lengths, etc.

\xzlNote{we better say 'input padding' instead of 'zero padding'. the latter exposes unecessary details and may trivialize the problem}

\paragraph{Redundancies in encoding} Inspecting the processing pipeline, firstly, there are redundancies in encoding processes. The audio buffer is fluctuating around the pre-defined length, 15 s as default. To accommodate the Whisper model requirement, the audio will be further padded into 30 s, as shown in ~\autoref{fig:intro} (b). The padding here cause substantial amount of redundant computation in the encoding stage. Considering the computational complexity of the transformer is $O(n^2 \cdot d + n \cdot d^2)$ ~\cite{vaswani2017attention}, the $d$ is the transformer model's dimension, and the $n$ is the input sequence length. Padding 15s audio to 30s makes $n$ increase by 2$\times$. This will result in encoding GFLOPS increase from $\sim$260 GFLOPS to $\sim$570 GFLOPS for encoding when applying whisper medium model. Simply erase the padding and input the audio with original length will result in collapse of model performance. To reduce the audio input length and the computation is a non-trivial problem that need new method design to solve.

\paragraph{Redundancies in decoding} Secondly, there are redundancies in decoding processes. The audio buffer get updated after each round but usually only has little difference between consecutive rounds. For most of the rounds, the audio buffer simply get extended for a certain short length. For some specific rounds, the audio buffer will get trimmed from the beginning. As a result, most of the transcription results in consecutive rounds share large overlaps, corresponds to redundancies in decoding processes. The beam search algorithm that Whisper model applies aggravate the problem. The beam search algorithm allows the model to explore more possible hypotheses to get the best one. But in the streaming system case, it is no longer necessary in some cases and will cause redundant computation.
The overlap part in the audio buffer is crucial although it cause redundancy: it provides context information for the model inference, which is critical for attention-based models~\cite{vaswani2017attention}. Simply removing the overlap and processing the new audio segment-wise will cause severe accuracy degradation, especially in the small chunk size cases. 

\xzlNote{should highlight why the two problems are nontrivial (e.g. they are ingrained in the algorihtm designs), and say that trival solutions would not work}

\xzlNote{e.g. some naive readers may wonder -- why we have to encode from the beginning of the audio every time? why we have to decode from the beginning of the audio every time?}

\xzlNote{you have to write defensively, forecasting where readers may come from}

% \subsection{The misalignment between speech workloads and hardware}
\subsection{SSP vs. modern hardware}

\xzlNote{the contents are there, but "under utilized resources" sound too plain (there are so many papers addressing this)
instead, frame it so that it is unique to the speech problem. 
the angle is that twofold opportunities:
 (a) that both encoding and decoding can be costly (cf item 3 in Intro), constituting significant portion of the overhead 
    (b) that the modern CPU is on a par with GPU in terms of decoding performance. (the contents you wrote). 
    also put your motivation table on.
}
The workloads in the SSP have diverse characteristics, so do the hardware processors available on modern edge devices.
The current generic system designs usually ignore the diversity, leading to misalignment between the workloads and the hardware processors and cause inefficiencies.

%\paragraph{Hardware on Mobile Devices is Heterogeneous}
%Modern mobile devices are equipped with capable CPUs for primary processing tasks, as well as auxiliary GPUs and DSPs for graphics and specialized signal processing ~\cite{chen2020deep}. Unlike devices with dedicated NVIDIA GPUs, mobile devices typically integrate GPUs within system-on-chips (SoCs), which, while less powerful, benefit from a shared memory architecture. Although mobile GPUs are rapidly evolving to support the increasing demands of AI applications, the performance gap between CPUs and GPUs on mobile devices remains relatively small compared to the pronounced difference seen in cloud computing clusters.

\paragraph{The SSP workloads have diverse characteristics}
SSP workloads, generally divided into encoding and decoding stages in each round, have varying characteristics that influence their preference for different processing units. 

\begin{itemize}
    \item expensive encoding....
    The encoding phase is highly parallelized, involving a one-pass encoding of 1,500 tokens which correspond to 30 seconds of audio. 
    \item decoding ... (cf intro writing)
    In contrast, decoding is a more sequential process, generating tokens one by one. In each decoding round, the decoder takes the previous round tokens (number depends on the beam size, which is usually 5) as the input and predicts the next token probabilities. 
\end{itemize}

As a result...
Due to its serialized feature, although the compute token counts could be much less than the encoding ($\sim$150 vs 1500), the latency of decoding is usually longer.

\input{tab-motivencdec}
\paragraph{opportunitijes in mapping SSP to CPU/GPU}
% \paragraph{Inadequate mapping of workloads on edge devices}
Due to the high parallelism characteristic, encoding strongly favors the GPU over the CPU; as shown in \autoref{tab:motivencdec}, experiments with Whisper’s medium model on Apple M2 chip show a 4.3$\times$ reduction in latency on the GPU. In contrast, the more sequential decoding process is more neutral to processor choices. Whisper medium model experiments on the same chip demonstrate a more modest latency improvement for decoding, with only a 1.1 - 1.5$\times$ difference. This indicate that the CPU resources could be useful for decoding workloads. However, the current SOTA system map all the workloads to GPU, leave the CPU mostly idle. 


==> overview__Felix_s_conflicted_copy_2024-12-04_.tex <==
% !TeX root = main.tex

\section{\sys{} Overview}
\label{sec:overview}
%\input{fig-pipeline}

%\xzlNote{"a \& b" bad; "a and b" good}

\subsection{The system model}
%\xzlNote{system model is about assumption of the hardware, software environment, use cases; not your own system, whic goes to 3.2}

We target edge hardware including mobile computers, smartphones, and embedded devices. 
Our system has minimum software dependencies, in particular no requirement for Python or any Python-based ML frameworks; 
it can be deployed to MacOS, Android, and Windows with ease. 
Once deployed, the system runs entirely on-device without requiring the cloud. 

Our system primarily runs on mobile GPU; 
it can opportunistically leverage idle CPUs through CPU/GPU pipelining for better performance. 
In case GPU is unavailable, our system falls back to CPU-only execution, albeit with higher latency and smaller models; in our experience, today's mobile CPUs are not powerful enough to run SOTA speech models in real time. 

% \sys{} augments an existing foundation models serving system with an additional offline hush word training framework and a hardware profiling \& pipeline planning framework. The offline hush word training framework is designed to train hush words for each of the foundation models. The hardware profiling and pipeline planning framework provides insights into hardware resources and further offers a system execution plan. The online foundation models serving system follows the scheme of the previous system, maintains an audio buffer, a transcript buffer, and confirms the results using LocalAgreement-2. \sys{} does not modify the model but separates the encoding and decoding workloads. It optimizes the execution of these two stages using hush word and beam pruning techniques. With an optional offline profiling for the threads pool allocations and a GPU-prioritized pipeline design, the workloads are mapped to heterogeneous processors.% to maximize hardware utilization.

\subsection{The operation}
\input{fig-pipeline}

Its primary use case is real-time transcription of daily conversations and peronsal speech. 
A typical scenario involves capturing streaming audio from a device's microphone and producing transcript tokens, which can be either displayed or sent to downstream applications like chat or online meeting applications.

The opertion is shown in ~\autoref{fig:pl}. 

\textbf{In offline development},
\sys{} requires to train special audio segments called hush word offline. 
We stress: only one hush word is needed for each foundation model (e.g. Whisper medium), 
it is a one-time effort. 
As an option, the offline development further profiles the target platform hardware to determine optimal thread allocations for CPU/GPU pipelining; without such profiling, the system runs model inference on GPU only. 

\textbf{In online operation}, 
the system ingests stremaing audio into the audio buffer continuously. 
Perodically, 
the sytem teaks a copy of the current audio buffer, runs model inference on it, and updates the transcript buffer.
Such periodic inferences are referred to as `rounds' as shown in the figture. 
Of each round: the computation of encoding, prompt prefilling, and word timestamping (using  dynamic time warping or DTW~\cite{bellman1959mathematical}  always runs on GPU; 
opportunistically, the ssytem oflfoading the 
the online policy engine offloads the decoding  to the CPU and forms a pipeline.  the results help maintain and update the transcript buffer. 
\sys{} applies LocalAgreement-2 ~\cite{Liu2020LowLatencySS}, %\xzlNote{cite; was this introduced?}, 
the transcript is confirmed when it occurs twice consecutively in the transcript buffer of two rounds. Based on the confirmed transcript and predefined threshold, the audio buffer is trimmed from the beginning to maintain around a certain length.  

With a user-defined step lengths (will be discussed in the later paragraph), %predefined time interval (step length \xzlNote{who determines it}) or execute eagerly \xzlNote{???}, 
\paragraph{Step length for system operations}, 
i.e., the interval between two consecutive inference rounds, 
impacts system operation as follows. 
When the step length is long, the system takes longer new audio segments, also has abundant time to finish processing the updated audio buffer once in each interval; in this case, a word's latency consists of the wait time (from the word's audio ingested into the buffer until the system starts the next inference round) and the system inference time on the audio buffer. %encoding time (the system encodes the whole audio buffer), and the decoding time (from decoding starts until the system emits the last token for this word, in auto regression). 
As the step length reduces, but still longer than the single round processing latencies in general (of which latencies could vary across processing rounds), the wait time in the per-word latency would decrease, therefore the per-word latency also decreases in general. 
As the step length drops below the single round processing latencies (in general), the system would not be able to catch up with the step length, it will run the model inference back-to-back and try to make the actually step length as short as possible.  %\xzlNote{finish}
We refer to this mode as ``best effort'' mode in the writing below. 
\xzlNote{can we say, there is a min "effective" step len a system can handle? if the step is shorter than that, the sytem will just take the most recent snapshot of audio buffer and process it}

%However, 
Note that lower step length tends to degrade model accuracy, this is because lower step length corresponds to shorter audio segment and less context information each round.
\xzlNote{in fact this is unclear to me: isnt' the input padded anyways? or is ti would be too easy for a token to pass the local-2 agreement check?}
A primary goal of \sys{} is to reduce the single round processing latencies and enable shorter step length and per token latency, without further accuracy degradation beyond the degradation caused by the shorter context.
%Therefore, a primary goal of \sys{} is to operate under shorter step lengths (which reduces per-word latency) while maintaining model accuracy.





\subsection{Applicability}
\sys{} supports encoder-decoder based speech foundation models. This paper focuses on SSP. The hush word is expected to also work on short audio transcription tasks and brings benefit. 

%Although the pipeline is an important design, the \sys{} can work in serialized mode and do all GPU / CPU execution. It is implemented on top of Whisper.cpp, which makes it easy to deploy to various mobile devices. 

\sys{} generally targets commodity edge devices like laptops, desktop computers, and smartphones. We expect these devices to be capable to execute some variants of the speech foundation models with an acceptable service latency. For more constrained devices, operating speech foundation models will be difficult and traditional on-device speech models may be a better choice. %but out of our scope. 
For cloud with better hardware, we expect our system still provides benefit. But the hush word may influence the batch processing, as it makes encoding workloads have irregular shapes.


==> recycle/recycle-intro.tex <==


Streaming speech processing (SSP) has become an essential task for real-time applications ~\cite{he2019streaming, moritz2020streaming, kannan2019large}. It enables the transcription of live audio inputs, facilitating its use in daily conversations ~\cite{xiong2017toward}, live-stream transcriptions~\cite{ranchal2013livestream}, online meetings~\cite{tur2008calo}, and various other scenarios.

\paragraph{Speech foundation models for speech processing}
Speech foundation models ~\cite{radford2023robust, peng2023reproducing} are end-to-end encoder-decoder transformer models that are trained on large volume of data. They are originally designed to deal with audio tasks with complete audio input. Recently, serving systems and pipelines are proposed to make them also work with SSP ~\cite{machavcek2023turning, ggerganov2022whispercpp}. The state-of-the-art system ~\cite{machavcek2023turning} maintain an audio buffer to provide context, and a transcript buffer to generate and confirm the result progressively. It periodically executes on the growing audio buffer, first do one-pass encoding then token-by-token decoding with beam search. 

Serving speech foundation model is resource-demanding, often requiring tens of GFLOPs of computation per second., as a result, the execution interval, which directly related to the streaming processing latency, can be a few seconds. Facing the constraints, the serving system is usually running on the cloud with powerful GPUs, which leads to cost, privacy and service accessability concerns ~\cite{microsoft2024azurewhisper}.

\paragraph{Problem \& approach}
This paper presents a runtime system to accelerate the speech foundation models performing SSP on resource-constrained mobile devices. 
\xzlNote{what are these? apple silicon? battery power devices, we can say}
The engine consists model execution and pipeline optimizations that specifically address unique challenges.
\subsection{The SSP system with Foundation model on mobile devices}


\xzlNote{hglight: 1500 tokens of encoding is a beast..... not seeming in LLM serving. like 1500 contexts... kinda unthinkable for mobile devices}

\xzlNote{has to say: the foundation modle is not trained in the straeming paradigm. trainign is inherently batch processed, for high efficiency.
this is crucial for scaling to colossoal data}

\paragraph{Challenge: redundancy in computation}
There are redundant computation when serving foundation models in SSP. To secure the high accuracy during the streaming processing, the state-of-the-art system adopted a process-and-confirm paradigm with LocalAgreement-2~\cite{Liu2020LowLatencySS}.
\xzlNote{need a title figure, batch, streaming (before) and streaming (ours)}
Because of these, the system involves making the foundation model transcribing the same audio segment multiple times and cause substantial redundancy in computation. 
\xzlNote{state hwy is this encessary}

In encoding, the audio buffer is length around 15s, while the foundation model usually requires a certain fixed input len, e.g. whisper model requires 30s. 
\xzlNote{explain why is this inherent to the model}
The common practice is to pad the audio to 30s to accommodate the model requirements, but suffer from the redundant computation. Simply erase the padding will cause the model output severe hallucinations and make the accuracy collapse ~\cite{Koenecke2024hallucinations}. 

In decoding, as the same audio segment will be transcribed multiple times, same piece of the transcript will be generated by token-by-token decoding multiple times, cause redundant computation. The commonly applied beam search algorithm ~\cite{hayes1976speech} which allows the model to explore multiple hypotheses in parallel aggravate the problem.

\paragraph{Our idea: audio tag and beam pruning}
For encoding, our insight is that the behavior of the foundation models can be manipulated by modifying the input with adversarial attack ~\cite{chen2020devil, raina2024mutingwhisperuniversalacoustic,raina2024controllingwhisperuniversalacoustic}. To this end, we propose audio tag, which is an audio adversarial segment trained to replace the redundant padding. With the audio tag as a suffix, the target foundation model can work with shorter input, with the computation reduced substantially.

For decoding, our insight is that the previous rounds results can be reused and assist the later rounds decoding ~\cite{wang2024turbochargespeechunderstandingpilot}. With the idea, we propose beam pruning, which reduce the beam search space with the guide of the previous results by pruning the hypotheses. 



\subsection{System serving on heterogeneous hardware}
\xzlNote{less important..., but still cna talk about it}

\paragraph{Challenge: insufficient utilization of heterogeneous hardware resources} 
The current mobile devices have heterogeneous processor designs. However, the resources are not being efficiently used. The state-of-the-art systems usually operate only on CPU or GPU~\cite{machavcek2023turning}. The optimal way to map the SSP workloads to all the available processors is still unclear. Naive approach will make the certain processor become bottleneck and even delay the whole process.

\paragraph{Our idea: new pipeline paradigm}
Our key insight is that different stage of the computation shows different characteristic. The encoding workload is much more parallel and has a strong preference on GPU while the decoding workload, due to its serial feature, can still gain good performance on CPU. 
\xzlNote{in fact well known - powerinfer. wahts' new? beam search? gpu stage also requires nontrivial cpu?}
To accommodate the characteristic of both the processors and the workloads in the pipeline, we reorganized the pipeline to offload part of the decoding workload to CPU to make the pipeline more compact and reduce the latency.

\subsection{Results and contributions}
We implement a system called \sys{}, atop various mobile platforms. We test \sys{} on long form audio datasets like TED-LIUM3. On SSP task, \sys{} delivers comparable accuracy with per-word latency as low as 600 ms. Compared to the popular foundation model SSP serving system, \sys{}'s on-device execution incurs 2-3x lower latency with little energy overhead.

Towards foundation model serving system for SSP, we contribute a first-of-its-kind foundation model serving system for SSP task specifically optimizes for embedded devices. It includes these contributions:

\begin{myitemize}


\item Audio hushtag, an adversarial audio tag for reducing the encoding computation of audio foundation models

\item Beam pruning, a reference-based method to reduce the beam search computation with the help of the previous results.


\item A new pipeline organization that make maximum utilization of the heterogeneous processors resources on the mobile devices. 
\end{myitemize}
	
We will make our model and code publicly available.	

==> recycle/recycle-intro2.tex <==
% !TeX root = main.tex

\section{Introduction}
\label{sec:intro}

Speech is a pervasive user interface. 
It is in particular useful to small embedded/IoT devices where hands free interactions are desirable. 
At the core of speech understanding are two ML tasks: 
transcribing the input to a textual sentence (e.g. ``xxxx''), 
called automatic speech recognition (ASR) \xzlNote{cite}; 
and further translating to a structured intent (e.g. ``yyyy''), 
called spoken language understanding (SLU) \xzlNote{cite}.
In this paper we refer both ASR and SLU as speech understanding (SU) tasks. 

Speech understanding has been challenging. 
Today, while narrated utterances (read after pre-defined text) can be transcribed or understood with high accuracy, 
utterances closer to human daily speeches still see a significant gap in accuracy \xzlNote{cite},
because of accents, lexical and grammar diversity, free-formed/irregular utterance, background noise...
%State-of-the-art (SOTA) 
Modern SU models typically embrace an encoder-decoder architecture \xzlNote{cite};
the decoder generates output tokens sequentially, called \textit{autoregression}. 
For instance, XXX has XXX parameters in XXXX transformer layers (XXX for encoding and YYY for decoding). 

To provide \su{} to embedded/IoT devices, 
the cloud and the devices offer complementary resources.
Cloud offers much richer compute resources as well as ease of model tuning and deployment. 
No wonder cloud execution is default to most commercial applications such as Google assistant and Amazon Alexa. \xzlNote{cite}
By comparison, 
on-device execution avoids network trips, which are vital to interactivity; 
it mitigates privacy concerns arising from 
the leak of speaker identity and sensitive entities and intents,
which are shown as real threats by recent work. \xzlNote{cite}
% the leak of speaker identity, biometrics; via speech transcripts -- semantics, sensitive entity, intents, etc. 


\begin{itemize}
\item Accuracy challenge: on 

\end{itemize}

\paragraph{Design goal: a device/cloud cascade for SU}
Like many AI tasks \xzlNote{cite}, 
speech understanding would benefit from device/cloud collaborative executions. 
The device processes input utterances with a simple \su{} model, 
and only offloads the inputs of low confidence to the cloud which runs a big model. 

\begin{comment}
To further reduce overhead for the device, a key optimization is \textit{early offload}: the device makes offload decisions based on partial processing of an input. Early offload for speech is supported by workload studies \xzlNote{cite}:most inputs are simple in acoustic variations and lexical structures, whereas fewer ones are rich and complex. The former inputs are likely resolved by the on-device model, while the latter inputs are worth the offload cost. 
\end{comment}

\wrxNote{
To further reduce overhead for the device, 
a key optimization is \textit{partial decoding}: the device makes offload decisions based on partial processing of an input. The local decoding can also be speedup by partial decoding results. The partial decoding take advantage of idle ingestion time in speech task to help with task which originally can only be done with complete data.
}

%We apply a proven execution paradigm (cite vision/camera tasks..) -- early offload -- to speech understanding tasks. 

\paragraph{Challenges}
While device/cloud executions and early offloading are well understood for other perception (AI) tasks \xzlNote{cite}, 
they remain largely unexplored for SU. 
The nature of speech and SU models raises unique challenges. 

% While this goal is reminiscent of prior offloading engines (esp for vision/camera tasks), 
%Not just a classification layer, but autoregressive sequence generation; 
%beam search, hypothesis ranking and scoring, etc. 
\wrxNote{Different from typical vision related task, SU tasks are generation tasks which usually involve autoregression. More specifically, beam search is usually adopted in these tasks. During the autoregression, the results will be generated token by token, and we will keep a certain beam size number of best hypothesis to help with improving robustness. This unique procedure make it hard to directly get basic understanding with linear classifier and intermediate encoder output.}

%streaming input / processing
\wrxNote{The streaming data ingestion is another unique feature in SU tasks. Dealing with partial data is a non-trivial problem.}


\textbf{Model pipeline...}

%early offload ... benefit is limited b/c it's latency bound

%offload to the cloud has to wait for the ingestion to complete... when the last audio segment is there

%so the network bandwidth is not a big deal

\wrxNote{The model pipeline and execution features are also worth inspect. The local and cloud model usually both require full length model to perform the decoding. On the cloud side, with the help of better hardware specification, the execution is quite fast. The offloading overhead mainly comes from data sanitizing and network communication. The local model have encoder and decoder part. The encoder execution is one-pass execution which have a relatively small runtime and large module size (memory footprint). The decoder execution is in autoregressing fashion, which have a long runtime and small module size.}

\textbf{Assessing confidence in autoregression}
To make offload decisions, 
the device needs to measure its confidence in (partial) processing results. 
This mechanism is called an \textit{offramp}. 
Prior work on early exit \xzlNote{cite} focused on classification tasks; 
%such as image classification; 
their offramps make tentative predictions, and the prediction entropy is used as the measure of confidence. 
This technique does not apply to SU:
(1) typically using an encoder-decoder architecture \xzlNote{cite}, 
the model generates output token by token, exploring multiple tentative sequences (called hypothesis) using complex beam search.
% in an autoregressive fashion \xzlNote{cite}. 
(2) the quality of final result is measured by XXX or word error rate (WER), not simply prediction accuracy. 
\wrxNote{(3) Generally speaking, prior research in the field has primarily focused on applying a simple classification layer to the intermediate representation of speech. However, this approach is insufficient in fully harnessing the underlying features, consequently leading to inaccurate estimations of the optimal strategy and offloading decisions in a local cloud collaboration scheme.}
% As we will show, the prediction entropy of individual token is a poor measure of the final outcome. 
As we will show, the per token entropy is a poor measure of the confidence. 
\wrxNote{As we will show, superfical feature like overall perplexing score is a poor measure of the confidence}

%\textbf{Early exit based on incomplete inputs}
\textbf{Early decoding based on incomplete inputs}
A unique aspect of SU is that the input (utterance) is streaming; 
the ingestion of an utterance takes seconds, comparable to the SU (inference) delay. 
Therefore, 
% it is beneficial to make early exit decisions \textit{before} the input is complete, 
% it is beneficial to make early exit \textit{before} the input is complete, 
it is beneficial to conduct partial decoding while the input is still being ingested, 
%allowing the device extra time to prepare the input for offloading (See Section XXX for details). 
allowing the device make early decision of offloading, also help with speeding up full length data decoding.
Existing early exit solutions do not apply here, as they decide based on partial processing of \textit{complete} inputs. \xzlNote{cite}
Furthermore, an encoder/decoder SU model expects an complete input in order to generate output tokens; experiments show that module customized for streaming data is needed in the confidence estimation of partial inputs.
%it was unclear how/if it can assess confidence in output based on partial inputs. 


\paragraph{\sys{}}
To this end, we present a runtime system. 
Executing on a client device, \sys{} manages the execution of ASR/SLU tasks.
It has three notable designs.


% A new architecture of device/cloud cascade. 
\textbf{A new device/cloud pipeline (cascade?) for SU: }
The device runs a series of SU models; 
\wrxNote{a modular model with multiple choices for each module to accommodate different input and scenarios}
for efficiency, they share much of weights and computations.
the first few ``early exit'' models attempt to output confidence and do not materialize output; 
\wrxNote{the first few exit points are off ramps that work with partial data. Through the decoding process, with dedicated predictors they can figure out the confidence of the data.}
the later one is for both \wrxNote{offload decision} and materializing output (in case of high confidence). 
A data sanitizing stage strips privacy information from data, if offload is decided. 
The whole cascade can be abstracted as a task graph. 


\textbf{Still useful:} restructure the encoder so it is (mostly) streaming; 
bottom layers convolution, a minimum number of top layers (attention) that require full input; \wrxNote{For partial data, the encoder is fully streaming. (Or it only uses the streaming part of the full encoder.)}
\xzlNote{merge}
We customize a modern speech model (encoder-decoder, attention based): 
so that bottom layers (closer to input) execute convolution which only require partial inputs, 
attention computation (which require complete inputs) is pushed to the top layers (closer to output). 
By deferring the attention computation, the model can generate meaningful intermediate results as input is ingested; it does not lose the benefit of attention (contextualization). 
The intermediate (encoding) results can be used to decode offramps. 


\textbf{Novel offramps for autoregression...}
It is a miniature decoder (transformer) that consumes partial model execution on partial input; 
based on encoder-decoder scores and language model perplexity, 
it predicts the final \wrxNote{local} confidence (if the on-device inference were to execute in full). 
We show how to train these offramps alongside the training of the on-device model. 
\textbf{Also:}
Partial inputs (short duration, inadequate information, incomplete beam search): hand crafted features, gradient boost, decision trees; 
Complete inputs (Bi-LSTM, sequence classification) \wrxNote{Current scheme: partial and full data both features extracted from beam search, Bi-LSTM prediction}

% We present a task scheduler (decision engine?)
\textbf{A scheduler for scheduling the cascade}: 
Question: which offramp to take; how to route inputs among local and cloud models?

Based on predictions made by offramps, 
the scheduler takes into account potential benefit (reduction in delays), potential accuracy gain, 
and routes the inputs among local models and the cloud. 
It orchestrates: 
local ingestion (streaming inputs); 
local encoding (multiple models, sharing?)
local offramps (tentative decoding, based on partial input)
local decoding (based on complete input)
offloading (data sanitizing/obfuscation), 




The scheduler abstracts the whole inference as a task graph, 
where nodes represent convolution, attention, off-ramps, and decoder; 
and edges capture data dependencies among nodes. 
The task scheduler starts from on-device execution path (inference), invokes offramps at various points, and judiciously switches to the offload path as it warrants. 
It makes scheduling decisions along two dimensions: input (should it consume more segments) and model layer (should it execute deeper layers). 
Furthermore, 
% it is resource conserving \xzlNote{cite}
it well utilizes resource for low delay: 
when encoding the streaming input cannot keep the device compute busy, 
the scheduler speculatively executes offload (sanitize tasks) even if it does not commit to offloading yet. 








\paragraph{Results}


\paragraph{Contributions}
We made three novel contributions. 

\begin{itemize}
\item An encoder-decoder model architecture (convolution on bottom layers; attention on top layers)
so that it suits early offloading on streaming (partial) inputs.

\item An off-ramp design (one-layer transformer) that predicts model confidence in generative output (autoregressive). Use a suite of optimizations: 
adaptive (?) beam width, language models, ...

\item A task scheduler: it judiciously inserts off-ramps into the task graph and switches from the on-device execution path to the offload path. 

\end{itemize}
	







 




==> recycle/recycle-motiv.tex <==
\section{Motivations}
\label{sec:motiv}

\subsection{SU needs device/cloud executions}

\xzlNote{moved here, merge}
Today, while narrated utterances (read after pre-defined text) can be transcribed or understood with high accuracy, 
utterances closer to human daily speeches still see a significant gap in accuracy \xzlNote{cite},
because of accents, lexical and grammar diversity, free-formed/irregular utterance, background noise...
%State-of-the-art (SOTA) 

it also offers ease of model tuning and deployment. 


On-device execution alone still lags behind the SOTA accuracy (satisfactory experience) significantly.
(1) User expectation for SU keeps increasing, as reflected by benchmark advance. 
(2) SOTA models large and expensive, based on encoder-decoder, transformers, pretrained foundation models, etc. 
This entails warrants cloud offloading as needed (for certain inputs). 

No wonder cloud execution is default to most commercial applications such as Google assistant and Amazon Alexa. \xzlNote{cite}
% the leak of speaker identity, biometrics; via speech transcripts -- semantics, sensitive entity, intents, etc. 



\subsection{What's unique about speech}

\textbf{also a primer...}
Paradigm shifts from Markov models, to RNNs (neural network sequence modeling). 
Recent advance in SSL (attention-based models, encoder-decoder architecture) is another major breakthrough. 

\paragraph{Speech processing different from video processing}
Speech data has long ingestion time. State of the art transformer model requires the full length data. 

\paragraph{privacy through sanitizing}
Recent work shows that speech privacy risk can be mitigates via  preprocessing (sanitize) before offloading, 
which, again, incurs significant processing delays (3x of the input duration). 

\paragraph{offloading: latency bound...}

\subsection{Analysis of SLU overhead}

Breakdown: input, encoding, decoding, ...

For parallelism, encoding can be segment by segment. (Convolution, to extract local features)
Only the top layer is transformer. 

Encoding is less likely the limiting factor. 
It is much cheaper than decoding, which must emit each token (subword) sequentially. 

at ingestion time, 




\subsection{Early offload or early exit?}


\xzlNote{moved here. to merge}
This paper has a simple goal: combine the best of both worlds (per-input, dynamic decision between on-device execution and offloading). 
In the spirit of (early filters), an edge device can resolve simple inputs (by executing a local model) without offloading (lower delays; lower model capacity); 
offload more difficult inputs after sanitizing them (higher delays; large model capacity). 



Early exit: materialize results with sufficiently high confidence that the results are correct

\begin{itemize}
\item Only possible when input becomes complete
\item Need to run the (expensive) decoder
\end{itemize}
	

Early offload: send to the cloud with sufficiently low confidence (low scores) that the results are correct


Why early exit: 

\subsection{Speech processing: what is unique}
Speech processing is a general field with many different tasks related to speech signal. There are ASR, which focus on transcripting speech signals; SLU which goes further and extract the intent and entities in the speech. There are also TTS which generate Speech signal with existing transcripts, ST which directly translate the speech to other language, etc. In this  project we focus on ASR and SLU tasks, which are fundamental tasks in the speech, also usually become frontend of a large related system.

The speech signal exhibits a distinctive nature. The original dataset comprises a one-dimensional vector that represents a sampled recording of the voice signal. For instance, when utilizing a 16k sampling rate, the resulting vector will possess a length of 16k, corresponding to one second of voice data. In the context of Automatic Speech Recognition (ASR) and Spoken Language Understanding (SLU), the prevailing and widely accepted approach involves employing an encoder-decoder based model. The data undergoes an initial frontend processing step, wherein it is transformed into a frequency spectrum. Subsequently, the processed data traverses through a convolutional neural network (CNN) and transformer-based encoder to further extract essential features. Ultimately, the transformer-based decoder, supplemented by an optional language model, decodes the data in a token-by-token manner, frequently utilizing beam search to aid in the decoding process.

Speech processing, quite different from image processing, is still an unsolved problem on mobile device. Speech signal usually have a long ingestion time, while image processing always have a frame of image ready to be processed. The image processing usually adopt CNN based model. However, the speech processing need transformer based model to achieve state-of-the-art accuracy. Transformer based models rely on the attention mechanism and have relatively large parameter sizes. As a consequence, the speech processing systems usually need to wait until the data finish ingestion and locate the model on a cloud server. The cloud-device communication and data offloading raise a concern on privacy loss. 


\begin{itemize}
\item Streaming input
\item Contextualization is vital to accuracy
\item Autoregression with beam search
\end{itemize}

\subsection{Speech data (signal): complexity and chance}
Speech data exhibits complexity from various perspectives. Some example factors are environmental variations, sentence lexical structure (inverted sentences, clauses, etc.), specialized terms and entities, etc. Moreover, individual differences in speech habits, including accents, pitch, speed and other factors, compound the complexities reflected in all the aforementioned aspects.

Data with varying complexity could also be processed with different deep learning models. For instance, large cloud-based models generally exhibit higher overall accuracy in ASR/SLU tasks. However, a closer examination reveals that a substantial portion of relatively simple data achieves similar accuracy with both large and small models, whereas more challenging data shows considerable different processing outcomes. 

Given this diversity in data complexity and the corresponding model requirements, there is a pressing need to develop methods that enable precise model selection and offloading decisions. This optimization is essential to conserve computational resources and minimize potential privacy risks.

\subsection{Speech related model: state-of-the-art and their constraints}
The present state-of-the-art models in the field of speech processing, namely Wav2vec2, HuBERT, conformer, and branchformer, can be conceptually divided into three main components: the CNN feature extraction part (Encoder.embed), the encoder transformer/CNN stack part (Encoder.stack), and the decoder part. Although these previous models (Wav2vec2, HuBERT, conformer, branchformer) demonstrate reasonable accuracy, they typically possess large model sizes and rely on GPU support for efficient inference, make them less suitable for deployment on mobile devices. Furthermore, in the case of transformer-based encoders, the requirement for full-length data ingestion introduces execution delays as the system awaits data ingestion completion before initiating any model execution decision.

At the same time, we could see that in these transformer-based model, there exist a parameter redundancy issue. E.g. the branchformer paper mentioned that some transformer block in the encoder.stack part play a less important role. Following the direction, we design a model group that trying to overcome the parameter redundancy issue, also provide modules that works on partial streaming data.

==> recycle/recyle-intro3.tex <==
% !TeX root = main.tex

\section{Introduction}
\label{sec:intro}

\xzlNote{merge this}
Note that pilot decoding, as a generic optimization technique, can be applied to other models without modifying their architectures. 


Speech is a pervasive user interface. 
It is in particular useful to small embedded/IoT devices where hands free interactions are desirable. 
At the core of speech understanding are two ML tasks: 
transcribing the input to a textual sentence (e.g. ``xxxx''), 
called automatic speech recognition (ASR) \cite{yu2016automatic}; 
and further translating to a structured intent (e.g. ``yyyy''), 
called spoken language understanding (SLU) \cite{de2007spoken}.
In this paper we refer both ASR and SLU as speech understanding (SU) tasks. 


\xzlNote{below: story has to update... two problems}
\begin{itemize}
\item local not fast enough (long delays -- motivate local path
\item local also needs to collaborate with cloud (for accuracy, limited model capacity -- motivate offload path
\end{itemize}

\paragraph{Basic paradigm: selective offloading}
SU has been a challenging AI task. 
To provide \su{} to embedded/IoT devices, 
the cloud/device collaboration is vital. 
The cloud can afford to execute large SU models, 
e.g. XXX has XXX parameters in XXXX transformer layers; 
on-device execution avoids network trips for low latency; 
, % which are vital to interactivity; 
it mitigates privacy concerns arising from the leak of speaker identity and sensitive entities and intents \cite{saade2019spoken} 
% which are shown as real threats by recent work. \xzlNote{cite}
Section XXX provides a detailed analysis. 
Therefore, we target selective offloading of SU: 
the device processes input utterances with a local \su{} model under resource constraints; 
% it can afford; 
it offloads the inputs for which the local inference is unlikely to yield correct results.


\paragraph{Unique aspects in speech:}
While offloading has been well explored for vision \cite{yao2020deep} and language \cite{lv2022walle} tasks, 
speech is different on multiple key aspects. 

(1) Slow, streaming input.
As a user utter, the device receives a stream of waveform segments. 
The duration of a spoken sentence is often several seconds, 
comparable to the local inference delay (also in seconds). 
Furthermore, the waveform size is small (less than hundreds of KBs ?? per input), 
making offloading the input latency-bound under typical network conditions. 
% Hence, it is vital to utilize compute source at the ingestion time. 

% (2) Context is crucial to inference accuracy. 
(2) Input context is crucial to accuracy. 
A common idea behind modern SU models is that 
% transcribing any portion of the input utterance should take into account the whole input (i.e. the context). 
any portion of the output should take into account the whole input (i.e. the context). 
For instance, in ``X Y Z'' the accurate prediction of X (or X'?) depends on Z. 
Accordingly, an SU model stacks transformer layers with all-to-all attention\cite{ashish2017attention}: 
%through the encoder, 
each input token (an acoustic frame) attends to all other input tokens; 
%through the decoder, 
each output token (a subword or word) attends to all input tokens and the output tokens generated prior to it. 
% is conditioned on all input tokens and the output tokens generated before it. 
As shown in prior work \cite{kuo2020interspeech} and also by us, 
lacking a complete context expected by the SU model, 
inference based on partial inputs results in significant word errors, e.g. .... , 

(3) Autoregressive output with beam search.  
A modern SU with an encoder-decoder architecture \cite{Jan2015NIPS}
generates the output sequence incrementally: 
% to generate each token in the sequence, it runs through the same set of layers which takes as input all the input tokens and the output tokens generated so far. 
to generate each output token, the model runs through the same set of decoding layers; 
the generation of the next token is conditioned on the previous output tokens and runs these layers again. 
To be robust against noisy input, the SU model further runs multiple autoregression processes, 
each generating a candidate output sequence (called a hypothesis). 
The model picks the best hypothesis as the final output. 
% after all autoregression concludes, the model outputs the best hypothesis. 
% As a result, the output is robust against input noises. 
See Section XXX for details. 
This \textit{autoregression} output contrasts to classification tasks (e.g. for images, for sentences) that send through an input through all model layers in one pass. 

% The above aspects raises two challenges. 
The aspects challenge our target execution in the following ways. 

\xzlNote{below map well to local path, offload path}

%\paragraph{Challenge 1: Load imbalance between ingestion/inference}
\paragraph{Challenge 1: how to utilize resources at the ingestion time}

\begin{itemize}
\item model arch expects complete input
\item send partial input through the model ... high errors
\end{itemize}

On-device execution suffers from a key inefficiency. 
% -- Load imbalance between ingestion/inference. 
Since both the encoder and decoder in an SU model expects a complete input,
the model poorly utilizes the computational resource during the ingestion time; 
% the input utterance is yet to be complete,  
as soon as the ingestion terminates (the input context becomes complete), 
the model spawns a surge of workload (encoding and then decoding), 
for which long delays are directly perceived by the user. 

% \paragraph{Challenge 2: Assessing confidence in autoregression}
\paragraph{Challenge 2: when to make offload decisions}

\begin{itemize}
\item ingestion time: input truncated (incomplete); 
\item during encoding: (intermediate encoding results) -- poor prediction of confidence
\item during/after decoding: too late (high delays). 
\end{itemize}

To decide whether to offload an input $x$, 
the device must predict $x$'s output confidence, i.e. 
how likely local inference of $x$ would yield an accurate answer.  
Preferably, the prediction itself should require \textit{shallow} processing of $x$,
leaving time for the subsequent offloading or local inference. 
A common approach for classification tasks (e.g. images or sentences)
%is to treats the entropy (uncertainty) in the classification posterior as the confidence, 
%where the classification can be the local model's final output 
%or based on its intermediate representations (i.e. ``early exit'' \xzlNote{cite}). 
is to assess confidence as the (un)certainty (i.e. entropy) in the model's intermediate output (the classification results of hidden layer activations) or the final output ( those of the final layer activations), 
This approach does not apply to autoregressive SU, 
for which the output is no longer one single posterior
but multiple hypotheses, each being a sequence of probabilistic tokens. 
Furthermore, these hypotheses are generated by not only one execution pass of model layers, but many repetitions of these model layers. 
Simple measures based on per-token probabilities, such as average token probability or sequence perplexity, poorly reflect the output confidence: 
because speech input is noisy, low probability tokens are not uncommon even in a high confidence output sequence. 
This will be shown in Section XXX. 

\xzlNote{here we don't motivate partial input much. but will sell it as a key idea}


\paragraph{Key ideas}

\xzlNote{local path} --- encoder, decoder

\xzlNote{offload path} -- offload timing, decisions

\begin{itemize}
% \item Late contextualization in the encoder. 
\item Model idea -- Late contextualization. 
We refactor an SU model so much of the encoding can be done at the ingestion time. 
Rather than computing all-to-all attention at each encoding layer, 
the bottom layers (closer to the input) compute only convolution, which extract local speech features;
the few top layers compute attention, which extract for global features with contextualization. 
By deferring the attention computation, 
the model can generate meaningful intermediate results as the input is being ingested; 
it still retains inference accuracy thanks to contextualization. 


\item System idea -- Pilot decoding. 
% During ingestion, use idle compute resources to make inference on the incomplete input. 
We further use ingestion-time resources to speed up full inference after the ingestion. 
During ingestion, use idle compute resources to make tentative inference. 
%The output cannot be materialized: 
%since the input is still incomplete, the output sequence is likely to contain substantial incorrect tokens near its end where the input is cutoff
%(e.g. ... ). 
% However, the beam search trace in pilot decoding can accelerate the full decoding, i.e. on the complete input after the ingestion: 
% However, the beam search trace in pilot decoding can accelerate the full decoding that consumes the complete input: 
% at low cost, the full decoding simply verify if the output token from pilot decoding are still valid, and only starts expensive beam search in case 
Despite that the output is likely to contain substantial incorrect tokens near its end,
it provides an explored path in beam search, which greatly accelerates the subsequent full decoding: 
to produce a token, the full decoding verifies if the pilot beam search trace are still valid and can be reused. 
The full decoding may directly output correct tokens from the pilot decoding (for speed) while only initiates expensive beam search in case it deviates from the pilot decoding is (for accuracy). 

Three techniques: 
\begin{itemize}
\item good predictor of final output confidence (how to eliminate the impact of high word errors?
\item warm up (?) or explored beam search  -- speed up
\item predict the final beam search depth (truncation beam search) --- speed up 
\end{itemize}

\item 
% Offramp for autoregression. 
% Autoregression confidence by 
% Modeling beam search history. 
Predicting confidence with beam search history. 
The key idea is not just looking at probabilities of individual tokens,
but rather how these probabilities change (distribute?) across decoding steps, 
their rankings, and the rankings of hypotheses. 
The rationale is rather than focusing on probabilities of individual output tokens,
we should consider their patterns across decoding steps as well as the rankings of hypotheses. 
While specific rules can be difficult to define, 
% To model the dynamics and map it to confidence, 
we construct a lightweight RNN model that predicts the SU accuracy based on the sequence of top-k tokens and hypotheses. 
% The predicted accuracy serves as the basis of offloading decisions.	




%Partial inputs (short duration, inadequate information, incomplete beam search): hand crafted features, gradient boost, decision trees; 
%Complete inputs (Bi-LSTM, sequence classification) 

\end{itemize}


\xzlNote{below could go to overview}

\paragraph{The system}
To this end, we present a runtime system. 
Executing on a client device, \sys{} manages the execution of ASR/SLU tasks.

As it ingests input segments, 
\sys{} executes the bottom encoder layers on them. 
Only computing convolutions, the execution is incremental, producing per-segment results $\{S_i\}, i=1..n$ that can be combined later.
Periodically, the device executes pilot inference with its idle resources: 
over all segments ingested so far: 
feeding $\{S_i\}, i=1..n$ to the top encoding layers that compute all-to-all attention;
this is followed by a small (cheap?) decoder that outputs tentative tokens via beam search. 
Based on the pilot inference, 
\sys{} predicts the final output confidence. 
Over the course of ingesting an input, 
\sys{} may execute pilot inference multiple times, 
each time on an increasingly longer input. 
The execution of pilot inferences is incremental:
each inference is based on the output of the previous inference. 

Once the ingestion is over, 
\sys{} makes the offloading decision by 
checking if the last pilot inference shows high confidence. 
Since this pilot inference is based on an input with length closest to the complete input, 
its confidence ....
Note that early offloading, i.e. before the ingestion completes, does not reduce the latency much: 
the device still has to offload the last segment  which takes one network trip. 
% offloading waveform is bound by network latency, 
% and the last segment would still take one network trip. 
If \sys{} decides not to offload and instead to make local inference, 
it finishes the encoding computation that was not yet done during the ingestion; 
it then executes the full decoding and accelerates it by exploiting pilot inference opportunistically. 


\xzlNote{moved here, merge}This improvement is tied to the preliminary decoding outcomes from pilot decoding, which subsequently assist in the complete length decoding process and adaptively reduces the beam size, thus eliminating unnecessary computations.

%\wrxNote{
%To further reduce overhead for the device, 
%a key optimization is \textit{partial decoding}: the device makes offload decisions based on partial processing of an input. The local decoding can also be speedup by partial decoding results. The partial decoding take advantage of idle ingestion time in speech task to help with task which originally can only be done with complete data.
%}

\paragraph{Results}
We implement \sys{} atop ESPnet \cite{watanabe2018espnet} and demonstrate it on mobile CPU and GPU of three embedded platforms. On two major SU tasks: ASR and SLU, \sys{} meets different target accuracy QoS while achieve state of the art low average RTF. We compare \sys{} against competitive baselines mentioned in previous works \cite{conformer-2020} \cite{peng2022branchformer} \cite{zhang2020transformer} as illustrated in Figure 1. Compared to local processing, \sys{} reaches a higher WER / IC with the same average RTF. Compared to cloud processing, \sys{} reaches same high WER / IC with x\% RTF reduction. Compared to the existing selective offload methods, with different target accuracy QoS, \sys{} shows y\% to z\% RTF reduction in average.

\paragraph{Contributions}
We made three novel contributions. 

\begin{itemize}
\item An encoder-decoder model architecture (convolution on bottom layers; attention on top layers)
so that it suits early offloading on streaming (partial) inputs.

\item Pilot decoding, a novel way to address resource underutilization during ingestion. 

\item An off-ramp design (one-layer transformer) that predicts model confidence in generative output (autoregressive). Use a suite of optimizations: 
adaptive (?) beam width, language models, ...

\item A task scheduler: it judiciously inserts off-ramps into the task graph and switches from the on-device execution path to the offload path. 

\end{itemize}
	







 




==> recycle_buffer/detail.tex <==
% !TeX root = main.tex

\section{\sys{}: Streaming SLU Processing}
In this section, we provide a detailed explanation of how the major components of \sys{} are designed.

\subsection{Late contextualization and corresponding model design}

We design / co-trained \& deployed an encoder-decoder architecture based model that have customized design on both encoder and decoder to accommodate the streaming and full length data processing. 

Encoder design:
\sys{} adopt a late contextualization encoder design. The bottom layers only contains convolution, allows the model to process the streaming data. The top layers only contains transformer based all-to-all attention computation that exploit the contextual information for full length data processing. During the data processing, the bottom layers processing result of partial data will be cached, and reused for full length processing to avoid re-calculation.

Decoder design:
\sys{} provides two different decoder design for pilot decoding and full length inference. The pilot decoding requires low RTF to reach high granularity, thus need cheaper decoder and beam search design. \sys{} provide 1 layer transformer decoder for pilot decoding, also limit the beam search length within 15 tokens. For full length decoding, to reach a better influence accuracy, \sys{} provide 1 layers transformer decoder, higher beam size and beam search token limit.

\subsection{Pilot decoding and full decoding speedup} 

We design an offramp that consist decoder and decoding tracker (tree structured data based lstm) to help with the data inspection and confidence estimation. During the data ingestion, the 

\subsection{Selective offloading}


\xzlNote{moved here, to merge}

\textbf{why use RNN to model the output confidence?}
The intuition is that the consistency of hypotheses rankings, etc. 
For example, low-probability tokens, if occur in sequence, 
often imply that the model lacks confidence in the semantic correctness for a whole output span; 
% often imply that a span in the output has flawed structure or semantics; 
by contrast, if such tokens are just dispersed, it could be due to acoustic noise and the output is still mostly correct. 
Another example, a hypothesis ranked at the top at every decoding step shows higher confidence 
than a hypothesis with rankings fluctuates across decoding steps. 
While the rules can be difficult to define manually, we take a learning approach: 
% To model the dynamics and map it to confidence, 
we construct a lightweight BiLSTM (RNN?) model that predicts the SU accuracy based on the sequence of beam search features (\xzlNote{vague?})
The predicted accuracy serves as the basis of offloading decisions.	


 \subsection{Confidence prediction with beam search history}

 We design a scheduler, which can pre-profile the device and decide the partial granularities of partial decoding. Another important work of it is to decide which partial decoding result to use,  
 

==> recycle_buffer/eval__Felix_Lin_s_conflicted_copy_2023-09-19_.tex <==
% !TeX root = main.tex


\section{Evaluation}
\label{sec:eval}
%We evaluate \sys{} to address different aspects of the streaming SLU processing system:
We answer a few question through the evaluation process:
\begin{myitemize}
    \item Can \sys{} reduce the latency with compatible accuracy?
    \item How much do different key designs count for the benefits we see?
    \item How does several system parameters (hardware specification, network condition) affect the system?
\end{myitemize}
\xzlNote{to revisit after the whole eval is written}

\subsection{Methodology}
\paragraph{Test platform}
As shown in Table~\ref{tab:platforms}, we test our device runtime 
on two embedded boards: 
board 1 with an efficiency-oriented processor, 
board 2 with a performance-oriented processor. 
Note that although our device runtime runs on CPUs, 
the idea of \sys{} applies to GPUs. 


\begin{comment}
with different CPU specifications. The board 1 have relatively low performance CPU, represent the common embedded devices. The board 2, on the other hand, have more capable CPU. Note that although in the evaluation part we only conduct experiments on CPU boards, \sys{} should also work with GPU and shows similar benefits.
\end{comment}

%\xzlNote{cloud...} %\xzlNote{How is the cloud latency measured...}
We estimate the cloud offloading delays from real-world ML serving. 
To do so, we develop a test harness: 
running on an x86 desktop, it sends each input waveform to the Azure speech service \xzlNote{cite} and records wall clock time. 
The test was running from the US east coast and requests to use east coast datacenters. 
For each input, we repeat the test on enterprise WiFi (bandwidth in 100s of MB and RTT in ms) and on 5G cellular networks, and use the average delay. 
Note that we do not use the outcome of Azure speech for accuracy evaluation, because we often find its accuracy inferior to the SOTA model (XXX) used by us. 

\begin{comment}
We choose speech API provided by Microsoft Azure as the cloud baseline. The cloud latency of each audio is measured by uploading it through the Azure speech transcribing API under school WIFI and 5G hot spot, and we measure the time between uploading and result comes out. This measurement is solely for latency measurement. We do not rely on the accuracy of the Azure service but instead use the state-of-the-art model accuracy as the benchmark for cloud processing accuracy.
\end{comment}
    
\input{tab-platforms}

\paragraph{Dataset and model training}
%We trained models in our system on the SLURP dataset, run all the baselines and our system on the same dataset and inspect the metrics we mentioned above.
We run our experiments on the SLURP dataset comprising 101.5 hours of speech \xzlNote{cite}, as summarized in \xzlNote{Table XXX}. 
SLURP is widely considered challenging: 
unlike many datasets of short commands (e.g. ``light on''), 
SLURP's utterances are more complex and closer to daily human speech
(e.g. ``\xzlNote{.....}''). 
Of all 141530 utterances, we use 119880 (85\%) for training and the rest for test, 
from which accuracy and latency are reported. 


\begin{comment}
Our experiments are based on the SLURP dataset, a renowned SLU corpus. This dataset comprises 141530 audio files from 211 speakers, totaling 101.5 hours. The dataset consists of short command utterances with an average length of ~2.6s. All the data is transcribted and labeled with 69 different intents. Model training is conducted using the training set that contains 119880 data points. Accuracy and Latency measurement is on the test set with 8211 data points, length ranging from 2.2s to 6.2s.
\end{comment}


%Total: 13K, we picked: 8K
%(\textbf{could be a problem}...)

\paragraph{Metrics}
\underline{Accuracy:}
We follow the common practice. 
For ASR, we report word error rate (WER). 
WER is the discrepancy between the model output and the gold (ground truth?) transcript, 
 defined as count of errors (substitutions, deletions, insertions) normalized by the sentence length.  
 For SLU, we report the intent classification accuracy. %\wrxNote{Redundent: In SLURP dataset, every data entry has a intent corresponding to scenario plus action. There are 69 different intents in the SLURP dataset.}

\underline{Latency:}
(1) We report user-perceive latency: 
the elapsed time from a user completing her utterance to our system emitting the complete SU result. This metric is also used by prior work \xzlNote{cite}. 
(2) We further report real time factor (RTF): 
the user-perceived latency normalized by the input utterance's duration. 


\begin{comment}
 the absolute latency of the system (wall clock...) as the time between the finish of the utterance speaking and the completion of the ASR result generation. This is the latency in the real world using case. Besides absolute latency, we also adopt real time factor (RTF), which equals to absolute latency (or system elapse time) normalized by corresponding speech duration, as a normalized latency metric.
%what knobs we tune? --- threshold. (need to justify how to tune this)
%compare the resultant delays... (user perceived)
\end{comment}

\paragraph{Baselines}
We compare our system with several designed baselines.
\begin{myitemize}
    \item \textit{All local}: The system processes all the data on the local model. It choose the best local model setting with compatible model size. We selects a few popular model structures like conformer, branchformer, CNN-RNNT, modify their hyperparameters to let them have the similar model size.

    \item \textit{All cloud}: The system blindly offloads all the data to the cloud side. We adopted a 2 pass end-to-end SLU model proposed in \wrxNote{cite}. The model includes one conformer based encoder, one conformer based deliberation encoder, two transformer based decoders for the first and the second pass, and a pretrained BERT language model.
    
    %\item \textit{Random offload}: The system randomly offloads data with certain probability to meet the accuracy requirement. \xzlNote{needed?}
    
    %\item \textit{LC offload}: The system adopts a linear classifier to predict the local WER/IC and decide whether offload or not.
    %\item \textit{PS offload}: The system offloads data base on its local perplexing score in decoding process.
    \item \textit{Ours}: In \sys{}, there are a customized late contextualized local model, the selective offloading offramp and the pilot decoding orchestrated together. 
\end{myitemize}

\underline{Methods}
We compare the latency of our system and baselines with the same set of target accuracy. We first measure the latency and accuracy of local and cloud baselines. Then we define a series of accuracy target between local baseline accuracy and cloud accuracy. By tuning the confidence threshold, we configure our system to meet the accuracy target, measure and compare the latency with baseline / previous methods.

\input{fig-e2e}

\subsection{End-to-End results}


\paragraph{Overall latency and accuracy}
\sys{} achieve latency as low as xxx / xxx ms with compatible \xzlNote{comparable} accuracy. (WER, IC). Among all the accuracy targets, \sys{} consistently achieves the lowest overall latency with 30\%-50\% latency reduction compare to baselines as demonstrated in Figure~\ref{fig:eval:e2e}.  

%\xzlNote{be brief, or delete}
%The overall benefits come from two aspects of innovation in offload pass (which focus on local-cloud collaboration) and local pass (which focus on local process speed up).

\xzlNote{vs cloud}
Compare to the \textit{All cloud} baseline, \sys{} reduces the overall latency by as much as 30\% with less than 0.25 intent classification accuracy decrease. This efficiency arises from \sys{} meticulously analyzing data during local processing and making selective decisions about data offloading to the cloud in the offloading pass.

\xzlNote{vs all local}
In comparison to the \textit{All local} baseline, our system achieves a 50\% runtime acceleration while maintaining the same accuracy target. When setting the latency target to match local processing, our system enhances performance with a 6\% reduction in WER and a 2.5\% improvement in IC. This is due to \sys{} conducting pilot decoding during ingestion, which accelerates the local decoding process.



\xzlNote{Utilization and efficiency ... two separate things. We probably should focus on the former. But needed? -- can wait}
\paragraph{Computational resource efficiency}
We evaluate computational resource efficiency on local processing. %Figure~\ref{fig:eval:resource}
Experiments show the detailed GPU utilization for an audio data in average for baseline (top) and ours (bottom). In general, our system can finish the decoding in a shorter time period. During the ingestion time, the baseline conformer model do nothing but wait. 
Our system periodically conduct pilot decoding bases on partial data, take better usage of the idle resources. After ingestion time, the baseline model starts the encoding-decoding process, take relatively long time to finish. Our system only need to do the transformer part encoding, save the encoding time. Decoding time is also much shorter, with the help of our adaptive beam size reduction method.

\subsection{Efficacy of our local execution path}


%\xzlNote{Figure 2 must be referenenced and discussed}
%\xzlNote{In particular the RNN-T baseline...}

The delay of the local processing can be divided into two parts: encoding and decoding. 


%\xzlNote{Since table 2 focuses on on-device model structure... it might be a bit weird to include our WER/IC here. how about: maybe show conformer/branchformer/rnn-t WER/IC in Fig 1, as local baselines?}

%\xzlNote{Table 2: consider a column graph?}

\input{tab-models}
%\input{fig-models}
\input{tab-models2}

%\paragraph{local path: Late contextualization model design}
\paragraph{Encoding speedup}

\textbf{--- BELOW --- }
Our encoder design finds a sweet spot between speed (from streaming processing) and accuracy (from contextualization). 

Compared to full attention encoders (Conformer and Branchformers), our encoding latency is much lower by 0.07 - 0.1 RTF. This is because we locate 3 attention layers at the end part (top part) of the encoder. This late contextualization technique help significantly reduce the non-streaming flops in the encoder. Compare to the baseline attention based models, our model reduce the non-streaming FLOPS by 80\%.
Meanwhile, we achieve accuracy comparable or even slightly higher accuracy because we still keep the necessary attention layers, which can utilize the context information and achieve high accuracy.

Compared to full streaming encoders (CNN+RNN-T), our accuracy is much higher by 7\% in WER and 4.2\% in IC thanks to careful introduction of contextualization  
Meanwhile, our encoding latency is only higher by 0.012 - 0.016 RTF. 
Such an encoding difference will be diminished by the difference in decoding delays

\textbf{--- ABOVE --- }

%Concerning the encoding time, our system reduces it by 60\% compares to the conformer-m baseline and branchformer baseline.
%This reduction is attributed to the fact that the baseline local processing with the conformer model employs a transformer-based encoder and decoder, which requires complete data lengths to initiate processing. 

%By contrast, our system customizes the encoder structure, designing the initial layers (6/9) to exclusively comprise CNN-based modules. 
%\textbf{This modification enables the system to accommodate streaming data.}
%Figure ~\ref{fig:eval:fig-models} shows the breakdown of the encoder FLOPS of local baseline models. Compares to the branchformer and conformer models, our model has significantly fewer FLOPS. 
%Although the CNN+RNNT model is a fully streaming model, it compromises a lot on accuracy. Overall, our encoder  design represents the most feasible approach for balancing the trade-off between latency and accuracy.

%We compare the model specification shown in Table~\ref{tab:eval:models}. 
%Compares to the conformer-M model and the Branchformer model, our customized model encoder achieves similar or higher WER/IC with lower non-streaming latency and a comparable \xzlNote{comparable} model size. 
%\textbf{The late contextualization allows the encoder to start processing earlier with streaming data.} 
%In the table, we break down the encoder FLOPS into two part: the "embed" part and the "encoders" part. The "embed" part only contains CNN layers and an embed layer, naturally supports the streaming processing. 
%However, the "encoders" part in the baseline conformer and branchformer encoders include a transformer block in each layer, preventing it from starting processing before ingestion is finished.
%On the other hand, our late contextualized encoder only have 3 transformer layers at the end, make the 66\% computation can be finished in a streaming fashion. 
%Overall, the late contextualization help the \sys{} save 80\% encoding non-streaming FLOPS compare to the baseline models. \xzlNote{I don't understand the 80\% argument...(it shoudl be the streaming argument, instead of saving of flops)} \wrxNote{change to non-streaming FLOPS. need further discussion on encoder operation}
%The model RTF break down of each part shows in table~\ref{tab:eval:models2} is also consistent with the FLOPS result.

\input{tab-pilot}
%\paragraph{local path: Pilot decoding and decoding speedup}

\paragraph{Decoding speedup}

%\xzlNote{moved here and merge}
Moreover, our system reduces the decoding time by 50\% compares to all the local baselines.
This improvement is tied to the preliminary decoding outcomes from pilot decoding, which subsequently assist in the complete length decoding process and adaptively reduces the beam size, thus eliminating unnecessary computations.


Pilot decoding plays an important role in \sys{} local processing speed up. We conduct experiments to compare the pilot decoding's significance and its performance in different granularity. the result shows in table~\ref{tab:eval:pilot}. 
Pilot decoding with 1 second granularity can help decrease the RTF by 50\% when fully local processing compares to all the local baselines 
%This benefit could decrease \xzlNote{when cloud offloading increase}, \xzlNote{the logic is twisted. need straight up} 
Compares to offloading bases on perplexing score without pilot decoding and acceleration, The \sys{} still shows ~40\% RTF decrease on WER target 0.12, when 70\% of the data has been offload to cloud.


\xzlNote{talk about how granularity impact local path}
%it can improve, but with diminish return... a few sentences on why
Smaller granularity can further decrease the decoding RTF. As seen in table ~\ref{tab:eval:pilot} a granularity of 0.3s exhibits the lowest decoding RTF among all the granularity. This is because a smaller granularity can make the partial data of pilot decoding more similar to the full length data, thus yielding a more accurate preliminary decoding result and aiding in the reduction of the beam size during the full decoding process.


%\xzlNote{discuss the tradeoff... which hinges on...}
The hardware specification determines the boundary of the granularity. The granularity need to be larger than the longest execution time of pilot decoding. For board 1 with a weaker CPU, the best granularity is 1s. For board 2, the better CPU enables the 0.3s granularity choice.


\subsection{Efficacy of our offloading path}

\input{tab-offload}

\sys{} inspects the data and selectively offloads some of them to the cloud side. 
\textbf{Our offloading strategies effectively estimates the local processing confidence of the data and selects data with low confidence to the cloud, reducing the latency by 0.03 RTF as compared to sampling with pilot decoding speed up.}
\xzlNote{talk about target, nontarget...} \wrxNote{I talk about it in the later part when talk about pilot decoding granularity, as the table 5 doesn't have target nontarget data}
Moreover, we offload 10\%-15\% less data compare to sampling for reaching same accuracy targets. The experiment results are shown in Table~\ref{tab:eval:offload}.

We have experimented with several methods for estimating local processing confidence. 
First, we demonstrate that a popular prior approach, which involves adopting a BERT-style linear classifier for confidence estimation in transformer-based models, does not yield favorable results in SU tasks. 
This approach was previously employed in DeeBERT, where classification layers were trained for each BERT layer to estimate the confidence and decide whether to exit processing midway. %\xzlNote{cite and explain in detail}. 
However, this method proves ineffective for SU tasks, as the linear layer cannot be effectively trained with the available data, resulting in identical output estimations for all inputs. We assume it is equivalent to random offloading. 

Furthermore, we find three methods that have similar efficacy in estimating confidence: the CNN-based method, the LSTM based method and the perplexing score based method. 
The CNN approach employs a CNN model that takes the encoder's intermediate output as input, while the LSTM model uses features extracted from the pilot decoding beam search as input. The perplexing score is directly calculated from the pilot decoding result. As shown in the table, these three approaches yield similar RTF at different WER target. Compares to random offloading, they reduce the RTF by approximately 15\% . We choose the perplexing score based method for its low complexity.


\xzlNote{about we using pilot decoding for offloading decisions...}
Note that the LSTM method and the perplexing score method mentioned above are based on pilot decoding results, thus the pilot decoding granularity also has impact on selective offloading. From the table~\ref{tab:eval:pilot} we can see that as granularity becomes finer, the decoding results can better assist in  selective offloading. We define the data as target data if local WER larger than cloud WER. When the WER target is set to be 0.12, 0.3s granularity help the 
\xzlNote{target/non target should be introduced formally}
offloading target / non target ratio goes to 1.45, while 2s granularity have ratio 1.05. When WER target is 0.15, 0.3s target / non target ratio goes to 2.23, while 2s have ratio 1.43


\subsection{Sensitivity to system parameters} 
\xzlNote{can wait}
\paragraph{Hardware specification}
Better local hardware with more powerful CPU can help with decreasing overall RTF for different accuracy target. Figure~\ref{fig:eval:e2e} shows experiments conducted on Jetson Orin Nano and Odroid N2+. Odroid N2+ have better CPU performance, thus get lower RTF on all the accuracy targets. However, the pilot decoding speed up ratio maintains the same among different devices. Besides, better CPU enables faster local pilot inference, make the granularity possible to be more finegrained. 

\paragraph{Network latency}
Worse network condition and longer network latency makes \sys{} have more significant RTF decrease compare to random offload. 

==> recycle_buffer/intro_0731.tex <==
% !TeX root = main.tex

\section{Introduction}
\label{sec:intro}

Speech is a pervasive user interface. 
It is in particular useful to small embedded/IoT devices where hands free interactions are desirable. 
At the core of speech understanding are two ML tasks: 
transcribing the input to a textual sentence (e.g. ``xxxx''), 
called automatic speech recognition (ASR) \xzlNote{cite}; 
and further translating to a structured intent (e.g. ``yyyy''), 
called spoken language understanding (SLU) \xzlNote{cite}.
In this paper we refer both ASR and SLU as speech understanding (SU) tasks. 

Speech understanding has been challenging. 
Today, while narrated utterances (read after pre-defined text) can be transcribed or understood with high accuracy, 
utterances closer to human daily speeches still see a significant gap in accuracy \xzlNote{cite},
because of accents, lexical and grammar diversity, free-formed/irregular utterance, background noise...
%State-of-the-art (SOTA) 
Modern SU models typically embrace an encoder-decoder architecture \xzlNote{cite};
the decoder generates output tokens sequentially, called \textit{autoregression}. 
For instance, XXX has XXX parameters in XXXX transformer layers (XXX for encoding and YYY for decoding). 

To provide \su{} to embedded/IoT devices, 
the cloud and the devices offer complementary resources.
Cloud offers much richer compute resources as well as ease of model tuning and deployment. 
No wonder cloud execution is default to most commercial applications such as Google assistant and Amazon Alexa. \xzlNote{cite}
By comparison, 
on-device execution avoids network trips, which are vital to interactivity; 
it mitigates privacy concerns arising from 
the leak of speaker identity and sensitive entities and intents,
which are shown as real threats by recent work. \xzlNote{cite}
% the leak of speaker identity, biometrics; via speech transcripts -- semantics, sensitive entity, intents, etc. 

%\paragraph{Opportunity of early offload}
\paragraph{Design goal: a device/cloud cascade for SU}
Like many AI tasks \xzlNote{cite}, 
speech understanding would benefit from device/cloud collaborative executions. 
The device processes input utterances with a simple \su{} model, 
and only offloads the inputs of low confidence to the cloud which runs a big model. 
To further reduce overhead for the device, 
a key optimization is \textit{early offload}: 
the device makes offload decisions based on partial processing of an input. 
Early offload for speech is supported by workload studies \xzlNote{cite}:
most inputs are simple in acoustic variations and lexical structures, 
whereas fewer ones are rich and complex. 
The former inputs are likely resolved by the on-device model, 
while the latter inputs are worth the offload cost. 

%We apply a proven execution paradigm (cite vision/camera tasks..) -- early offload -- to speech understanding tasks. 

\paragraph{Challenges}
While device/cloud executions and early offloading are well understood for other perception (AI) tasks \xzlNote{cite}, 
they remain largely unexplored for SU. 
The nature of speech and SU models raises unique challenges. 

% While this goal is reminiscent of prior offloading engines (esp for vision/camera tasks), 
Not just a classification layer, but autoregressive sequence generation; 
beam search, hypothesis ranking and scoring, etc. 

streaming input / processing


\textbf{Model pipeline...}

early offload ... benefit is limited b/c it's latency bound

offload to the cloud has to wait for the ingestion to complete... when the last audio segment is there

so the network bandwidth is not a big deal


\textbf{Assessing confidence in autoregression}
To make offload decisions, 
the device needs to measure its confidence in (partial) processing results. 
This mechanism is called an \textit{offramp}. 
Prior work on early exit \xzlNote{cite} focused on classification tasks; 
%such as image classification; 
their offramps make tentative predictions, and the prediction entropy is used as the measure of confidence. 
This technique does not apply to SU:
(1) typically using an encoder-decoder architecture \xzlNote{cite}, 
the model generates output token by token, exploring multiple tentative sequences (called hypothesis) using complex beam search.
% in an autoregressive fashion \xzlNote{cite}. 
(2) the quality of final result is measured by XXX or word error rate (WER), not simply prediction accuracy. 
\wrxNote{(3) Generally speaking, prior research in the field has primarily focused on applying a simple classification layer to the intermediate representation of speech. However, this approach is insufficient in fully harnessing the underlying features, consequently leading to inaccurate estimations of the optimal strategy and offloading decisions in a local cloud collaboration scheme.}
% As we will show, the prediction entropy of individual token is a poor measure of the final outcome. 
As we will show, the per token entropy is a poor measure of the confidence. 
\wrxNote{As we will show, superfical feature like overall perplexing score is a poor measure of the confidence}

\textbf{Early exit based on incomplete inputs}
A unique aspect of SU is that the input (utterance) is streaming; 
the ingestion of an utterance takes seconds, comparable to the SU (inference) delay. 
Therefore, 
% it is beneficial to make early exit decisions \textit{before} the input is complete, 
% it is beneficial to make early exit \textit{before} the input is complete, 
it is beneficial to make early exit while the input is still being ingested, 
allowing the device extra time to prepare the input for offloading (See Section XXX for details). 
Existing early exit solutions do not apply here, as they decide based on partial processing of \textit{complete} inputs. \xzlNote{cite}
Furthermore, an encoder/decoder SU model expects an complete input in order to generate output tokens; 
it was unclear how/if it can assess confidence in output based on partial inputs. 


\paragraph{\sys{}}
To this end, we present a runtime system. 
Executing on a client device, \sys{} manages the execution of ASR/SLU tasks.
It has three notable designs.


% A new architecture of device/cloud cascade. 
\textbf{A new device/cloud pipeline (cascade?) for SU: }
The device runs a series of SU models; 
\wrxNote{a modular model with multiple choices for each module to accommodate different input and scenarios}
for efficiency, they share much of weights and computations
the first few ``early exit'' models attempt to output confidence and do not materialize output; 
\wrxNote{the first few exit points are off ramps that }
the later one is for both early exits and materializing output (in case of high confidence). 
A data sanitizing stage strips privacy information from data, if offload is decided. 
The whole cascade can be abstracted as a task graph. 


\textbf{Still useful:} restructure the encoder so it is (mostly) streaming; 
bottom layers convolution, a minimum number of top layers (attention) that require full input; 
\xzlNote{merge}
We customize a modern speech model (encoder-decoder, attention based): 
so that bottom layers (closer to input) execute convolution which only require partial inputs, 
attention computation (which require complete inputs) is pushed to the top layers (closer to output). 
By deferring the attention computation, the model can generate meaningful intermediate results as input is ingested; it does not lose the benefit of attention (contextualization). 
The intermediate (encoding) results can be used to decode offramps. 


\textbf{Novel offramps for autoregression...}
It is a miniature decoder (transformer) that consumes partial model execution on partial input; 
based on encoder-decoder scores and language model perplexity, 
it predicts the final confidence (if the on-device inference were to execute in full). 
We show how to train these offramps alongside the training of the on-device model. 
\textbf{Also:}
Partial inputs (short duration, inadequate information, incomplete beam search): hand crafted features, gradient boost, decision trees; 
Complete inputs (Bi-LSTM, sequence classification)

% We present a task scheduler (decision engine?)
\textbf{A scheduler for scheduling the cascade}: 
Question: which offramp to take; how to route inputs among local and cloud models?

Based on predictions made by offramps, 
the scheduler takes into account potential benefit (reduction in delays), potential accuracy gain, 
and routes the inputs among local models and the cloud. 
It orchestrates: 
local ingestion (streaming inputs); 
local encoding (multiple models, sharing?)
local offramps (tentative decoding, based on partial input)
local decoding (based on complete input)
offloading (data sanitizing/obfuscation), 




The scheduler abstracts the whole inference as a task graph, 
where nodes represent convolution, attention, off-ramps, and decoder; 
and edges capture data dependencies among nodes. 
The task scheduler starts from on-device execution path (inference), invokes offramps at various points, and judiciously switches to the offload path as it warrants. 
It makes scheduling decisions along two dimensions: input (should it consume more segments) and model layer (should it execute deeper layers). 
Furthermore, 
% it is resource conserving \xzlNote{cite}
it well utilizes resource for low delay: 
when encoding the streaming input cannot keep the device compute busy, 
the scheduler speculatively executes offload (sanitize tasks) even if it does not commit to offloading yet. 








\paragraph{Results}


\paragraph{Contributions}
We made three novel contributions. 

\begin{itemize}
\item An encoder-decoder model architecture (convolution on bottom layers; attention on top layers)
so that it suits early offloading on streaming (partial) inputs.

\item An off-ramp design (one-layer transformer) that predicts model confidence in generative output (autoregressive). Use a suite of optimizations: 
adaptive (?) beam width, language models, ...

\item A task scheduler: it judiciously inserts off-ramps into the task graph and switches from the on-device execution path to the offload path. 

\end{itemize}
	







 




==> recycle_buffer/motiv_0808.tex <==
\section{Motivations}
\label{sec:motiv}

\subsection{SU needs device/cloud executions}

\xzlNote{moved here, merge}
Today, while narrated utterances (read after pre-defined text) can be transcribed or understood with high accuracy, 
utterances closer to human daily speeches still see a significant gap in accuracy \xzlNote{cite},
because of accents, lexical and grammar diversity, free-formed/irregular utterance, background noise...
%State-of-the-art (SOTA) 

it also offers ease of model tuning and deployment. 


On-device execution alone still lags behind the SOTA accuracy (satisfactory experience) significantly.
(1) User expectation for SU keeps increasing, as reflected by benchmark advance. 
(2) SOTA models large and expensive, based on encoder-decoder, transformers, pretrained foundation models, etc. 
This entails warrants cloud offloading as needed (for certain inputs). 

No wonder cloud execution is default to most commercial applications such as Google assistant and Amazon Alexa. \xzlNote{cite}
% the leak of speaker identity, biometrics; via speech transcripts -- semantics, sensitive entity, intents, etc. 



\subsection{What's unique about speech}

\textbf{also a primer...}
Paradigm shifts from Markov models, to RNNs (neural network sequence modeling). 
Recent advance in SSL (attention-based models, encoder-decoder architecture) is another major breakthrough. 

\paragraph{Speech processing different from video processing}
Speech data has long ingestion time. State of the art transformer model requires the full length data. 

\paragraph{privacy through sanitizing}
Recent work shows that speech privacy risk can be mitigates via  preprocessing (sanitize) before offloading, 
which, again, incurs significant processing delays (3x of the input duration). 

\paragraph{offloading: latency bound...}

\subsection{Analysis of SLU overhead}

Breakdown: input, encoding, decoding, ...

For parallelism, encoding can be segment by segment. (Convolution, to extract local features)
Only the top layer is transformer. 

Encoding is less likely the limiting factor. 
It is much cheaper than decoding, which must emit each token (subword) sequentially. 

at ingestion time, 




\subsection{Early offload or early exit?}


\xzlNote{moved here. to merge}
This paper has a simple goal: combine the best of both worlds (per-input, dynamic decision between on-device execution and offloading). 
In the spirit of (early filters), an edge device can resolve simple inputs (by executing a local model) without offloading (lower delays; lower model capacity); 
offload more difficult inputs after sanitizing them (higher delays; large model capacity). 



Early exit: materialize results with sufficiently high confidence that the results are correct

\begin{itemize}
\item Only possible when input becomes complete
\item Need to run the (expensive) decoder
\end{itemize}
	

Early offload: send to the cloud with sufficiently low confidence (low scores) that the results are correct


Why early exit: 

\subsection{Speech processing: what is unique}
Speech processing is a general field with many different tasks related to speech signal. There are ASR, which focus on transcripting speech signals; SLU which goes further and extract the intent and entities in the speech. There are also TTS which generate Speech signal with existing transcripts, ST which directly translate the speech to other language, etc. In this  project we focus on ASR and SLU tasks, which are fundamental tasks in the speech, also usually become frontend of a large related system.

The speech signal exhibits a distinctive nature. The original dataset comprises a one-dimensional vector that represents a sampled recording of the voice signal. For instance, when utilizing a 16k sampling rate, the resulting vector will possess a length of 16k, corresponding to one second of voice data. In the context of Automatic Speech Recognition (ASR) and Spoken Language Understanding (SLU), the prevailing and widely accepted approach involves employing an encoder-decoder based model. The data undergoes an initial frontend processing step, wherein it is transformed into a frequency spectrum. Subsequently, the processed data traverses through a convolutional neural network (CNN) and transformer-based encoder to further extract essential features. Ultimately, the transformer-based decoder, supplemented by an optional language model, decodes the data in a token-by-token manner, frequently utilizing beam search to aid in the decoding process.

Speech processing, quite different from image processing, is still an unsolved problem on mobile device. Speech signal usually have a long ingestion time, while image processing always have a frame of image ready to be processed. The image processing usually adopt CNN based model. However, the speech processing need transformer based model to achieve state-of-the-art accuracy. Transformer based models rely on the attention mechanism and have relatively large parameter sizes. As a consequence, the speech processing systems usually need to wait until the data finish ingestion and locate the model on a cloud server. The cloud-device communication and data offloading raise a concern on privacy loss. 


\begin{itemize}
\item Streaming input
\item Contextualization is vital to accuracy
\item Autoregression with beam search
\end{itemize}

\subsection{Speech data (signal): complexity and chance}
Speech data exhibits complexity from various perspectives. Some example factors are environmental variations, sentence lexical structure (inverted sentences, clauses, etc.), specialized terms and entities, etc. Moreover, individual differences in speech habits, including accents, pitch, speed and other factors, compound the complexities reflected in all the aforementioned aspects.

Data with varying complexity could also be processed with different deep learning models. For instance, large cloud-based models generally exhibit higher overall accuracy in ASR/SLU tasks. However, a closer examination reveals that a substantial portion of relatively simple data achieves similar accuracy with both large and small models, whereas more challenging data shows considerable different processing outcomes. 

Given this diversity in data complexity and the corresponding model requirements, there is a pressing need to develop methods that enable precise model selection and offloading decisions. This optimization is essential to conserve computational resources and minimize potential privacy risks.

\subsection{Speech related model: state-of-the-art and their constraints}
The present state-of-the-art models in the field of speech processing, namely Wav2vec2, HuBERT, conformer, and branchformer, can be conceptually divided into three main components: the CNN feature extraction part (Encoder.embed), the encoder transformer/CNN stack part (Encoder.stack), and the decoder part. Although these previous models (Wav2vec2, HuBERT, conformer, branchformer) demonstrate reasonable accuracy, they typically possess large model sizes and rely on GPU support for efficient inference, make them less suitable for deployment on mobile devices. Furthermore, in the case of transformer-based encoders, the requirement for full-length data ingestion introduces execution delays as the system awaits data ingestion completion before initiating any model execution decision.

At the same time, we could see that in these transformer-based model, there exist a parameter redundancy issue. E.g. the branchformer paper mentioned that some transformer block in the encoder.stack part play a less important role. Following the direction, we design a model group that trying to overcome the parameter redundancy issue, also provide modules that works on partial streaming data.

==> recycle_buffer/motiv_0812.tex <==
\section{Motivations}
\label{sec:motiv}

\subsection{SU needs device/cloud executions}

\xzlNote{moved here, merge}
Today, while narrated utterances (read after pre-defined text) can be transcribed or understood with high accuracy, 
utterances closer to human daily speeches still see a significant gap in accuracy \xzlNote{cite},
because of accents, lexical and grammar diversity, free-formed/irregular utterance, background noise...
%State-of-the-art (SOTA) 

it also offers ease of model tuning and deployment. 


On-device execution alone still lags behind the SOTA accuracy (satisfactory experience) significantly.
(1) User expectation for SU keeps increasing, as reflected by benchmark advance. 
(2) SOTA models large and expensive, based on encoder-decoder, transformers, pretrained foundation models, etc. 
This entails warrants cloud offloading as needed (for certain inputs). 

No wonder cloud execution is default to most commercial applications such as Google assistant and Amazon Alexa. \xzlNote{cite}
% the leak of speaker identity, biometrics; via speech transcripts -- semantics, sensitive entity, intents, etc. 



\subsection{What's unique about speech}

\textbf{also a primer...}
Paradigm shifts from Markov models, to RNNs (neural network sequence modeling). 
Recent advance in SSL (attention-based models, encoder-decoder architecture) is another major breakthrough. 

\paragraph{Speech processing different from video processing}
Speech data has long ingestion time. State of the art transformer model requires the full length data. 

\paragraph{privacy through sanitizing}
Recent work shows that speech privacy risk can be mitigates via  preprocessing (sanitize) before offloading, 
which, again, incurs significant processing delays (3x of the input duration). 

\paragraph{offloading: latency bound...}

\subsection{Analysis of SLU overhead}

Breakdown: input, encoding, decoding, ...

For parallelism, encoding can be segment by segment. (Convolution, to extract local features)
Only the top layer is transformer. 

Encoding is less likely the limiting factor. 
It is much cheaper than decoding, which must emit each token (subword) sequentially. 

at ingestion time, 




\subsection{Early offload or early exit?}


\xzlNote{moved here. to merge}
This paper has a simple goal: combine the best of both worlds (per-input, dynamic decision between on-device execution and offloading). 
In the spirit of (early filters), an edge device can resolve simple inputs (by executing a local model) without offloading (lower delays; lower model capacity); 
offload more difficult inputs after sanitizing them (higher delays; large model capacity). 



Early exit: materialize results with sufficiently high confidence that the results are correct

\begin{itemize}
\item Only possible when input becomes complete
\item Need to run the (expensive) decoder
\end{itemize}
	

Early offload: send to the cloud with sufficiently low confidence (low scores) that the results are correct


Why early exit: 

\subsection{Speech processing: what is unique}
Speech processing is a general field with many different tasks related to speech signal. There are ASR, which focus on transcripting speech signals; SLU which goes further and extract the intent and entities in the speech. There are also TTS which generate Speech signal with existing transcripts, ST which directly translate the speech to other language, etc. In this  project we focus on ASR and SLU tasks, which are fundamental tasks in the speech, also usually become frontend of a large related system.

The speech signal exhibits a distinctive nature. The original dataset comprises a one-dimensional vector that represents a sampled recording of the voice signal. For instance, when utilizing a 16k sampling rate, the resulting vector will possess a length of 16k, corresponding to one second of voice data. In the context of Automatic Speech Recognition (ASR) and Spoken Language Understanding (SLU), the prevailing and widely accepted approach involves employing an encoder-decoder based model. The data undergoes an initial frontend processing step, wherein it is transformed into a frequency spectrum. Subsequently, the processed data traverses through a convolutional neural network (CNN) and transformer-based encoder to further extract essential features. Ultimately, the transformer-based decoder, supplemented by an optional language model, decodes the data in a token-by-token manner, frequently utilizing beam search to aid in the decoding process.

Speech processing, quite different from image processing, is still an unsolved problem on mobile device. Speech signal usually have a long ingestion time, while image processing always have a frame of image ready to be processed. The image processing usually adopt CNN based model. However, the speech processing need transformer based model to achieve state-of-the-art accuracy. Transformer based models rely on the attention mechanism and have relatively large parameter sizes. As a consequence, the speech processing systems usually need to wait until the data finish ingestion and locate the model on a cloud server. The cloud-device communication and data offloading raise a concern on privacy loss. 


\begin{itemize}
\item Streaming input
\item Contextualization is vital to accuracy
\item Autoregression with beam search
\end{itemize}

\subsection{Speech data (signal): complexity and chance}
Speech data exhibits complexity from various perspectives. Some example factors are environmental variations, sentence lexical structure (inverted sentences, clauses, etc.), specialized terms and entities, etc. Moreover, individual differences in speech habits, including accents, pitch, speed and other factors, compound the complexities reflected in all the aforementioned aspects.

Data with varying complexity could also be processed with different deep learning models. For instance, large cloud-based models generally exhibit higher overall accuracy in ASR/SLU tasks. However, a closer examination reveals that a substantial portion of relatively simple data achieves similar accuracy with both large and small models, whereas more challenging data shows considerable different processing outcomes. 

Given this diversity in data complexity and the corresponding model requirements, there is a pressing need to develop methods that enable precise model selection and offloading decisions. This optimization is essential to conserve computational resources and minimize potential privacy risks.

\subsection{Speech related model: state-of-the-art and their constraints}
The present state-of-the-art models in the field of speech processing, namely Wav2vec2, HuBERT, conformer, and branchformer, can be conceptually divided into three main components: the CNN feature extraction part (Encoder.embed), the encoder transformer/CNN stack part (Encoder.stack), and the decoder part. Although these previous models (Wav2vec2, HuBERT, conformer, branchformer) demonstrate reasonable accuracy, they typically possess large model sizes and rely on GPU support for efficient inference, make them less suitable for deployment on mobile devices. Furthermore, in the case of transformer-based encoders, the requirement for full-length data ingestion introduces execution delays as the system awaits data ingestion completion before initiating any model execution decision.

At the same time, we could see that in these transformer-based model, there exist a parameter redundancy issue. E.g. the branchformer paper mentioned that some transformer block in the encoder.stack part play a less important role. Following the direction, we design a model group that trying to overcome the parameter redundancy issue, also provide modules that works on partial streaming data.

==> scripts/Makefile <==
# batch convert all .pptx files in a directory to .pdf  
# files and crop them. 
# 
# to be used in conjunction with ppt.vbs, which converts
# a .pptx file into a pdf. 
#
# usage: copy this file and ppt.vbs to figs/ and run make
# there
#
# environment: win 10 cmd
#

docobjects := $(patsubst %.docx,%.pdf,$(wildcard *.docx)) $(patsubst %.dox,%.pdf,$(wildcard *.dox))
pptobjects := $(patsubst %.pptx,%.pdf,$(wildcard *.pptx))

current_dir  := $(shell cd)

all : check_overlap $(docobjects) $(pptobjects) 

	
docx : $(docobjects)

pptx : $(pptobjects)

clean :
	del /Q $(docobjects) $(pptobjects)

check_overlap :
	@echo "$(current_dir)"
		
		
%.pdf.uncrop : %.docx
	"c:\Windows\SysWOW64\cscript.exe" "$(scriptDir)\docx.vbs" "$(current_dir)\$^" "$(current_dir)\$@"

%.pdf.uncrop : %.dox
	"c:\Windows\SysWOW64\cscript.exe" "$(scriptDir)\docx.vbs" "$(current_dir)\$^" "$(current_dir)\$@"

%.pdf.uncrop : %.pptx
	"c:\Windows\SysWOW64\cscript.exe" "$(scriptDir)\ppt.vbs" "$(current_dir)\$^" "$(current_dir)\$@"

%.pdf: %.pdf.uncrop
	"$(scriptDir)\bin\pdfcrop.exe" $^ $@
	
	
.PHONY: check_overlap all docx pptx

==> scripts/bin/pdfcrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__


==> summary__Felix_s_conflicted_copy_2023-11-30_.tex <==
% !TeX root = main.tex
\section{Conclusions}
We present \sys{}, a novel system for fast speech processing in SU tasks. \sys{} contributes late contextualization, beam collapse/ termination, and CTC leap for local execution; 
and confidence estimation for selective offloading. 
%The former allows \sys{} accelerate local execution while the latter one enables users to better trade-off the accuracy and latency. 
All optimizations combined, \sys{} speeds up its local path by 2x and reduces the offloading needs by 2x in its offloading path.



%We present \sys{}, a novel system for fast speech processing in SU tasks. \sys{} contributes late contextualization, beam collapse, beam search early termination and ctc leap techniques for local execution and confidence estimation techniques for hybrid execution collaborating with cloud service. The former allows \sys{} accelerate local execution while the latter one enables users to better trade-off the accuracy and latency. With the techniques, the \sys{} can reduce 2x for local execution, and reduce 50\% or more offloading and cloud service queries for hybrid execution. 

==> tab-ctcleap.tex <==
% !TeX root = main.tex
%\begin{table*}[t]
%    \centering
%    \caption{Platforms in evaluation for cloud and local side. Cloud side has GPU support while local side only runs on CPU}
%    \includegraphics[width=0.48\textwidth{}]{./figs/tab_platforms}
%    \label{tab:platforms}
%\end{table*}
\begin{algorithm}[t!]
    %\centering
        \includegraphics[width=0.42\textwidth{}]{./figs/ctcleap}
        \caption{Algorithm modified with CTC leap for CTC prefix scoring speedup. 
        The \sethlcolor{green}\hl{highlighted} part is our modification to reuse the calculation in pilot inference and skip part of the calculation. The remaining parts are the same as the hybrid CTC/attention algorithm \cite{watanane2017hybridctc}.}
        \label{tab:ctcleap}
\end{algorithm}


==> tab-glossary.tex <==
% !TeX root = main.tex
%\begin{table*}[t]
%    \centering
%    \caption{Platforms in evaluation for cloud and local side. Cloud side has GPU support while local side only runs on CPU}
%    \includegraphics[width=0.48\textwidth{}]{./figs/tab_platforms}
%    \label{tab:platforms}
%\end{table*}
\begin{table}[t]
    %\centering
        \includegraphics[width=0.48\textwidth{}]{./figs/glossary}
        \caption{A glossary of terms used in the paper}
        \centering
        \label{tab:glossary}
\end{table}


==> tab-modelflops.tex <==
% !TeX root = main.tex
%\begin{table*}[t]
%    \centering
%    \caption{Platforms in evaluation for cloud and local side. Cloud side has GPU support while local side only runs on CPU}
%    \includegraphics[width=0.48\textwidth{}]{./figs/tab_platforms}
%    \label{tab:platforms}
%\end{table*}
\begin{table}[t!]
    \centering
        \includegraphics[width=0.48\textwidth{}]{./figs/modelflops}
        \caption{Our local encoder executes mostly streaming FLOPs, 
        for which latency can be hidden behind IO; 
        doing so does not compromise the final accuracy. 
        FLOPs numbers normalized to 1 second of input.
        Our local execution path incurs lower latencies (reported as RTF) as compared to other on-device models. % for both encoding and decoding,
        }
        \label{tab:modelflops}
\end{table}


==> tab-offloadingstrategy.tex <==
% !TeX root = main.tex
\begin{table}[t]
    \centering
        \includegraphics[width=0.48\textwidth{}]{./figs/offloadingstrategy}
        \caption{Our offloading strategies based on sequence modeling outperform  \textit{NaiveHybrid} (random selection) and DeeBERT (sequence classification, failing to produce useful results). 
        In the experiment, we tune $\theta$ and $\alpha$ to meet WER goals and compare delays and offloading ratio}
        \label{tab:offloadingstrategy}
\end{table}


==> tab-pilotspeedup.tex <==
% !TeX root = main.tex
%\begin{table*}[t]
%    \centering
%    \caption{Platforms in evaluation for cloud and local side. Cloud side has GPU support while local side only runs on CPU}
%    \includegraphics[width=0.48\textwidth{}]{./figs/tab_platforms}
%    \label{tab:platforms}
%\end{table*}
\begin{table}[t]
    \centering
        \includegraphics[width=0.48\textwidth{}]{./figs/pilotspeedup}
        \caption{Pilot inference reduces the end-to-end delay. 
        % The benefits come from speeding up our local path (Ours-NoOffload) as well as the offloading path (Ours-Offload-X),
        It benefits our local-only execution (Ours-NoOffload) as well as our hybrid executions (Ours-Offload-X),
        making the latter's offloading more selective.}
        %\label{tab:pilotspeedup}
        \label{tab:psu}
\end{table}

==> tab-slurpdataset.tex <==
\begin{table}[t!]
    \centering
        \includegraphics[width=0.45\textwidth{}]{./figs/slurpdataset}
        \caption{Overview of SLURP dataset for SU tasks}
        \label{tab:slurpdataset}
\end{table}

